Benchmarking Evaluation Metrics for Code-Switching Automatic Speech Recognition

Code-switching poses a number of challenges and opportunities for multilingual automatic speech recognition. In this paper, we focus on the question of robust and fair evaluation metrics. To that end, we develop a reference benchmark data set of code-switching speech recognition hypotheses with human judgments. We define clear guidelines for minimal editing of automatic hypotheses. We validate the guidelines using 4-way inter-annotator agreement. We evaluate a large number of metrics in terms of correlation with human judgments. The metrics we consider vary in terms of representation (orthographic, phonological, semantic), directness (intrinsic vs extrinsic), granularity (e.g. word, character), and similarity computation method. The highest correlation to human judgment is achieved using transliteration followed by text normalization. We release the first corpus for human acceptance of code-switching speech recognition results in dialectal Arabic/English conversation speech.

==> sections/introduction.tex <==
\section{Introduction} % all of page 1
Code-switching (CS) is common in multi-cultural and multi-lingual societies, where speakers are bilingual and often switch between languages, such as Arabic-English (Arabizi), Hindi-English (Hinglish) and Spanish English (Spanglish), among many others, which can be seen as high-resource \textit{mono-language} in these language pairs \cite{ERR+18, HVA20}. In other cases like in South Africa, there are eleven spoken languages, of which Zulu and Xhosa are the most widely spoken, remarkably, in a single spoken utterance, a speaker may switch between Afrikaans, Xhosa and English \cite{reitmaier2022opportunities}. In cases where code-switching happens in language-pairs with different scripts, rendering the transcription of code-switched accurately is important. However, transcribing code-switched speech is often not straight-forward, and can be inconsistent, leading to the same word being transcribed using different writing scripts \cite{SS18}.

Several socio-linguistic factors affect CS, due to which it is not uniform across language pairs \cite{dougruoz2021survey}. \cite{gamback2016comparing} define the Code-Mixing Index to measure the complexity of CS across languages and find that languages such as Nepali-English and Mandarin-English have a very high amount of switching compared to languages such as Dutch-Turkish in the Social Media corpora they study.

%placed here to appear on second page
\begin{table*}[h]
\centering
 \includegraphics[width=\textwidth]{tables/fun_example-cropped.pdf}
 \label{table:fun_example}
 \caption{This example shows a hypothesis (H), the minimal edit (ME) annotation, as well as the ArzEn transcription reference (R). We denote annotation decisions as substitution (S), insertion (I), deletion (D), or acceptance (A) for words having different forms across H and ME. %We show CER/WER(ME,H) and CER/WER(R,H) reflecting the ground truth error of human post-editing as well as the CER and WER calculated between hypotheses and references. 
 In this example, CER and WER reductions are seen for minimal edits annotations over reference due to cross-transcription (segments 1, 2, 3, and 4) and unstandardized orthography (segments 9, 13, 14, and 16) issues.% (and unclear segment due to high speaking rate (segment 10)).
 }
 %\textcolor{red}{@Ahmed: Please let me know if this is okay or if you'd like to do it differently}}\textcolor{red}{@Amir: please explain what are ME, A, }
\end{table*}

Automatic Speech Recognition for Code-switching is a well studied problem \cite{SCR+19} with studies in several language pairs on acoustic modeling, language modeling and novel system architectures. In code-switched language pairs with different scripts, there is a tendency to cross-transcribe words that creates a large number of homophones in the data, leading to challenges in training and evaluation. Cross-transcription is particularly challenging in languages that have a high amount of borrowing, as it is not always clear which language a word belongs to, and hence, which script to transcribe it in. \cite{SS18} propose a modified WER metric based on mapping both languages into the pronunciation space, which leads to improvements in accuracy and evaluation. \cite {ERR+18} propose a transliteration-based WER metric by transliterating mixed-script utterances into a single script. However, these techniques can also lead to false positives when there are words in the two languages that sound the same but have a different meaning. It also has limitations in cases where different part of the word written in different script. e.g, the word \textbf{\<آرت>ficial}, which is \textbf{artificial} in English script or \textbf{\<آرتفيشيال> } in Arabic script. 
Thanks to word-pieces \cite{chowdhury2021towards}, we may expect partial transcription in code-switching ASR results. %simple has not been recognized in English script  or Arabic script thanks to word-pieces, which may allows these cases in multi-lingual code-switching ASR results .

This work builds upon previous contributions from \cite{ERR+18} that uses transliteration approach to normalize transcribed speech. The authors demonstrated the robustness of the proposed approach on several Indic languages%from Google Voice Search traffic with significant gains in with 10\% relative ASR improvement
. Previous researchers have also investigated handling the problem of non-standardized orthography for Dialectal Arabic ASR evaluation. \cite{AMR15} proposed the use of Multi-Reference Word Error Rate to allow for a wider coverage of different spelling variants. \cite{AKH19} investigated approaches to reduce spelling variations, which included normalization and following the Conventional Orthography for Dialectal Arabic (CODA) \cite{HDR12} guidelines to spell words, as well as relying on morphologically abstracted forms obtained from different tokenization schemes and lemmatization. In our paper, we investigate various methods that go beyond orthographic transliteration methods. We explore lexical and phonetic representations for evaluation, and study various weighted edit-distance methods and semantic similarity evaluation. We believe that this is the first study on human acceptability for code-switching speech recognition. The contributions of this paper are as follows:

\begin{itemize}[noitemsep]

\item We release the first corpus for human acceptance for code-switching speech recognition;
\item We introduce phone similarity edit distance (PSD) and show its correlation with human acceptance;
\item We propose a novel approach to use machine translation on both hypotheses and reference and report results using semantic evaluation to overcome the cross-transcription challenge.
\end{itemize}

\begin{comment}

* not all CS pairs are equal in complexity
* magic example
* challeneges of CS evaluation

* generalizability to other language pairs


\begin{figure}[t!]
    \centering
%    \includegraphics{}
\begin{tabular}{c|c}
     XXXX &  \\
     XXXX & \\
     XXXX &  \\
     XXXX & \\
     XXXX &  \\
     XXXX & \\
     
\end{tabular}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

%while WER is currently the de facto metric used for assessing speech recognition systems, several researchers have discussed its limitations \cite{}. Such limitations are further exacerbated in the case of code-switching, due to the possibility of code-switching segments to be written in either scripts, especially in the case of loanwords. In Figure/Table\ref{}, we show how CER and WER are both inadequate performance indicators, where many words and characters are incorrectly penalized, leading to a CER and WER that is double that achieved by human judgment.


\begin{figure}
  \includegraphics[width=\linewidth]{figures/cs_fun_example.png}
  \caption{(fun cs) Example demonstrating the difference between WER/CER and human assessment using minimal correction.}
  \label{fig:fun_cs}
\end{figure}
\end{comment}

%"researchers have argued the non-suitability of the WER metric for the evaluation of ASR systems for downstream tasks such as spoken language understanding (SLU) and information retrieval. The reason is that the WER works at the surface level and does not include any syntactic and semantic knowledge." \cite{Roy21}. Despite the great advances in ASR systems over the past year, "the means of evaluating the quality of a speech recognition system has remained mostly unchanged. WER is still the de facto standard metric for ASR system assessment."

==> sections/introduction_shortened_v1.tex <==
\section{Introduction} % all of page 1
Code-switching (CS) is common in multi-cultural and multi-lingual societies, where speakers are bilingual and often switch between languages, such as Arabic-English, Hindi-English (Hinglish) and Spanish English (Spanglish), among many others, which can be seen as high-resource \textit{mono-language} in these language pairs \cite{ERR+18, HVA20}. In other cases like in South Africa, there are eleven spoken languages, of which Zulu and Xhosa are the most widely spoken, remarkably, in a single spoken utterance, a speaker may switch between Afrikaans, Xhosa and English \cite{reitmaier2022opportunities}. 

Automatic Speech Recognition (ASR) for CS is a well studied problem \cite{SCR+19} with studies in several language pairs on acoustic modeling, language modeling and novel system architectures. In code-switched language pairs with different scripts, there is a tendency to cross-transcribe words that creates a large number of homophones in the data, leading to challenges in training and evaluation.
%%In cases where code-switching happens in language-pairs with different scripts, 
Rendering the transcription of code-switched accurately is important, however, it is often not straight-forward, and can be inconsistent, leading to the same word being transcribed using different writing scripts \cite{SS18}. Cross-transcription is particularly challenging in languages that have a high amount of borrowing, as it is not always clear which language a word belongs to, and hence, which script to transcribe it in. 
%Several socio-linguistic factors affect CS, due to which it is not uniform across language pairs \cite{dougruoz2021survey}. \cite{gamback2016comparing} define the Code-Mixing Index to measure the complexity of CS across languages and find that languages such as Nepali-English and Mandarin-English have a very high amount of switching compared to languages such as Dutch-Turkish in the Social Media corpora they study.
%placed here to appear on second page
\begin{table*}[h]
\centering
 \includegraphics[width=0.95\textwidth]{tables/fun_example-cropped.pdf}
 \label{table:fun_example}
 \caption{This example shows a hypothesis (H), the minimal edit (ME) annotation, as well as the ArzEn transcription reference (R). We denote annotation decisions as substitution (S), insertion (I), deletion (D), or acceptance (A) for words having different forms across H and ME. %We show CER/WER(ME,H) and CER/WER(R,H) reflecting the ground truth error of human post-editing as well as the CER and WER calculated between hypotheses and references. 
 In this example, CER and WER reductions are seen for minimal edits annotations over reference due to cross-transcription (segments 1, 2, 3, and 4) and unstandardized orthography (segments 9, 13, 14, and 16) issues.% (and unclear segment due to high speaking rate (segment 10)).
 }
 %\textcolor{red}{@Ahmed: Please let me know if this is okay or if you'd like to do it differently}}\textcolor{red}{@Amir: please explain what are ME, A, }
\end{table*}
\cite{SS18} propose a modified WER metric based on mapping both languages into the pronunciation space, which leads to improvements in accuracy and evaluation. \cite {ERR+18} propose a transliteration-based WER metric by transliterating mixed-script utterances into a single script. However, these techniques can also lead to false positives when there are words in the two languages that sound the same but have a different meaning. It also has limitation in cases where different part of the word written in different script. e.g, the word \textbf{\<آرت>ficial}, which is \textbf{artificial} in English script or \textbf{\<آرتفيشيال> } in Arabic script. 
Thanks to word-pieces \cite{chowdhury2021towards}, we may expect partial transcription in CS ASR results. %simple has not been recognized in English script  or Arabic script thanks to word-pieces, which may allows these cases in multi-lingual code-switching ASR results .

This work builds upon previous contributions from \cite{ERR+18} that uses transliteration approach to normalize transcribed speech. The authors demonstrated the robustness of the proposed approach on several Indic languages%from Google Voice Search traffic with significant gains in with 10\% relative ASR improvement
. Previous researchers have also investigated handling the problem of non-standardized orthography for Dialectal Arabic ASR evaluation. \cite{AMR15} proposed the use of Multi-Reference Word Error Rate to allow for a wider coverage of different spelling variants. \cite{AKH19} investigated approaches to reduce spelling variations, which included normalization and following the Conventional Orthography for Dialectal Arabic (CODA) \cite{HDR12} guidelines to spell words, as well as relying on morphologically abstracted forms obtained from different tokenization schemes and lemmatization. In our paper, we investigate various methods that go beyond orthographic transliteration methods. We explore lexical and phonetic representations for evaluation, and study various weighted edit-distance methods and semantic similarity evaluation. We believe that this is the first study on human acceptability for code-switching speech recognition. The contributions of this paper are as follows:

\begin{itemize}[noitemsep]

\item We release the first corpus for human acceptance for code-switching speech recognition;
\item We introduce phone similarity edit distance (PSD) and show its correlation with human acceptance;
\item We propose a novel approach to use machine translation on both hypotheses and reference and report results using semantic evaluation to overcome the cross-transcription challenge.
\end{itemize}

\begin{comment}

* not all CS pairs are equal in complexity
* magic example
* challeneges of CS evaluation

* generalizability to other language pairs


\begin{figure}[t!]
    \centering
%    \includegraphics{}
\begin{tabular}{c|c}
     XXXX &  \\
     XXXX & \\
     XXXX &  \\
     XXXX & \\
     XXXX &  \\
     XXXX & \\
     
\end{tabular}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

%while WER is currently the de facto metric used for assessing speech recognition systems, several researchers have discussed its limitations \cite{}. Such limitations are further exacerbated in the case of code-switching, due to the possibility of code-switching segments to be written in either scripts, especially in the case of loanwords. In Figure/Table\ref{}, we show how CER and WER are both inadequate performance indicators, where many words and characters are incorrectly penalized, leading to a CER and WER that is double that achieved by human judgment.


\begin{figure}
  \includegraphics[width=\linewidth]{figures/cs_fun_example.png}
  \caption{(fun cs) Example demonstrating the difference between WER/CER and human assessment using minimal correction.}
  \label{fig:fun_cs}
\end{figure}
\end{comment}

%"researchers have argued the non-suitability of the WER metric for the evaluation of ASR systems for downstream tasks such as spoken language understanding (SLU) and information retrieval. The reason is that the WER works at the surface level and does not include any syntactic and semantic knowledge." \cite{Roy21}. Despite the great advances in ASR systems over the past year, "the means of evaluating the quality of a speech recognition system has remained mostly unchanged. WER is still the de facto standard metric for ASR system assessment."

==> sections/introduction_shortened_v2.tex <==
\section{Introduction} % all of page 1
% Code-switching (CS) is common in multi-cultural and multi-lingual societies, where speakers are bilingual and often switch between languages, such as Arabic-English, Hindi-English (Hinglish) and Spanish English (Spanglish), among many others, which can be seen as high-resource \textit{mono-language} in these language pairs \cite{ERR+18, HVA20}. In other cases like in South Africa, there are eleven spoken languages, of which Zulu and Xhosa are the most widely spoken, remarkably, in a single spoken utterance, a speaker may switch between Afrikaans, Xhosa and English \cite{reitmaier2022opportunities}. 

% modified by shammur


% The term 
Code-switching (CS) refers to the phenomenon where the speaker switches between two languages within the same discourse.  
In spontaneous speech, CS is very common and yet highly unpredictable and difficult to model. %With the advent of multilingualism, there has been an increasing interest in code-switching (CS) automatic speech recognition (ASR) \cite{SCR+19}. 
Automatic Speech Recognition (ASR) for CS is a well studied problem \cite{SCR+19} conducted in several language pairs on acoustic modeling, language modeling and novel system architectures. 

In code-switched language pairs with different scripts, there is a tendency to cross-transcribe words that creates a large number of homophones in the data, leading to challenges in training and evaluation. 
Rendering the CS transcription accurately is important, however, is often not straight-forward, and can be inconsistent, leading to the same word being transcribed using different scripts \cite{SS18}. Cross-transcription is particularly challenging in languages having a high amount of borrowing words, as it is not always clear which language a word belongs to, and hence, which script to transcribe it in. 
%Several socio-linguistic factors affect CS, due to which it is not uniform across language pairs \cite{dougruoz2021survey}. \cite{gamback2016comparing} define the Code-Mixing Index to measure the complexity of CS across languages and find that languages such as Nepali-English and Mandarin-English have a very high amount of switching compared to languages such as Dutch-Turkish in the Social Media corpora they study.
%placed here to appear on second page

\begin{table*}[h]
\centering
 \includegraphics[width=0.9\textwidth]{tables/fun_example_shortened-cropped.pdf}
 \label{table:fun_example}
 \caption{This example shows a hypothesis (H), the minimal edits annotation (ME), the ArzEn transcription reference (R), and their Buckwalter transliterations \cite{Buckwalter:2002:buckwalter} (R\_BW, H\_BW, and ME\_BW). We denote annotation decisions (A-Decision) as substitution (S), insertion (I), deletion (D), or acceptance (A) for words having different forms across H and ME. %We show CER/WER(ME,H) and CER/WER(R,H) reflecting the ground truth error of human post-editing as well as the CER and WER calculated between hypotheses and references. 
 In this example, CER and WER reductions are seen for minimal edits annotations over reference due to cross-transcription (segments 1, 2, 3, and 4) and unstandardized orthography (segments 9 and 13) issues.% (and unclear segment due to high speaking rate (segment 10)).
 }
 %\textcolor{red}{@Ahmed: Please let me know if this is okay or if you'd like to do it differently}}\textcolor{red}{@Amir: please explain what are ME, A, }
\end{table*}

Investigating the ideal ASR performance metric for CS, \cite{SS18} propose a modified WER metric based on mapping both languages into the pronunciation space, which leads to improvements in accuracy and evaluation. \cite {ERR+18} propose a transliteration-based WER metric by transliterating mixed-script utterances into a single script. The authors demonstrated the robustness of the proposed approach on several Indic languages. 
% keep it, if space allows, else commented
% \begin{comment}
Moreover, researchers have also investigated techniques for handling the problem of non-standardized orthography.% for Dialectal Arabic ASR evaluation.
\cite{AMR15} proposed the use of Multi-Reference Word Error Rate to allow for a wider coverage of different spelling variants for Dialectal Arabic ASR evaluation. 
Whereas, \cite{AKH19} investigated approaches to reduce spelling variations, which included normalization and following the Conventional Orthography for Dialectal Arabic (CODA) \cite{HDR12} guidelines to spell words, as well as relying on morphologically abstracted forms obtained from different tokenization schemes and lemmatization. 
% \end{comment}

Even though the aforementioned studies \cite {ERR+18,SS18} showed improved CS ASR performance, these techniques can also lead to false positives when there are words in the two languages that sound the same but have a different meaning. It also has limitation in cases where different part of the word written in different script. e.g, the word \textbf{\<آرت>ficial}, which is \textbf{artificial} in English script or \textbf{\<آرتفيشيال> } in Arabic script. 
Thanks to word-pieces \cite{chowdhury2021towards}, we may expect partial transcription in CS ASR results. %simple has not been recognized in English script  or Arabic script thanks to word-pieces, which may allows these cases in multi-lingual code-switching ASR results .

% Previous researchers have also investigated handling the problem of non-standardized orthography for Dialectal Arabic ASR evaluation. \cite{AMR15} proposed the use of Multi-Reference Word Error Rate to allow for a wider coverage of different spelling variants. \cite{AKH19} investigated approaches to reduce spelling variations, which included normalization and following the Conventional Orthography for Dialectal Arabic (CODA) \cite{HDR12} guidelines to spell words, as well as relying on morphologically abstracted forms obtained from different tokenization schemes and lemmatization.

This work builds upon previous contributions from \cite{ERR+18} and \cite{SS18} and investigate various methods that go beyond orthographic transliteration methods. 
In this study, we explore lexical and phonetic representations for evaluation, and study various weighted edit-distance methods and semantic similarity evaluation. 
We designed a guideline and developed a reference human acceptability corpus (HAC) -- quantifying the human judgements in terms of minimal editing of ASR hypothesis. We evaluate a large number of metric in correlation with human judgements. 
We believe that this is the first study on human acceptability for CS speech recognition. 

\noindent The contributions of this paper are as follows:
\setlength\itemsep{-0.1em}
\setlist[itemize]{noitemsep, topsep=-0.1pt}
\begin{itemize} %[noitemsep]

\item We design, develop and publicly release the first corpus for human acceptance for CS speech recognition;%\footnote{Data download link will be available upon paper acceptance.}

% \item We release the first corpus for human acceptance for code-switching speech recognition;%\footnote{Data download link will be available upon paper acceptance.}
\item We introduce phone similarity edit distance (PSD) and show its correlation with human acceptance;
\item We propose a novel approach to use machine translation on both hypotheses and reference and report results using semantic evaluation to overcome the cross-transcription challenge.
\end{itemize}

\begin{comment}

* not all CS pairs are equal in complexity
* magic example
* challeneges of CS evaluation

* generalizability to other language pairs


\begin{figure}[t!]
    \centering
%    \includegraphics{}
\begin{tabular}{c|c}
     XXXX &  \\
     XXXX & \\
     XXXX &  \\
     XXXX & \\
     XXXX &  \\
     XXXX & \\
     
\end{tabular}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

%while WER is currently the de facto metric used for assessing speech recognition systems, several researchers have discussed its limitations \cite{}. Such limitations are further exacerbated in the case of code-switching, due to the possibility of code-switching segments to be written in either scripts, especially in the case of loanwords. In Figure/Table\ref{}, we show how CER and WER are both inadequate performance indicators, where many words and characters are incorrectly penalized, leading to a CER and WER that is double that achieved by human judgment.


\begin{figure}
  \includegraphics[width=\linewidth]{figures/cs_fun_example.png}
  \caption{(fun cs) Example demonstrating the difference between WER/CER and human assessment using minimal correction.}
  \label{fig:fun_cs}
\end{figure}
\end{comment}

%"researchers have argued the non-suitability of the WER metric for the evaluation of ASR systems for downstream tasks such as spoken language understanding (SLU) and information retrieval. The reason is that the WER works at the surface level and does not include any syntactic and semantic knowledge." \cite{Roy21}. Despite the great advances in ASR systems over the past year, "the means of evaluating the quality of a speech recognition system has remained mostly unchanged. WER is still the de facto standard metric for ASR system assessment."

==> sections/introduction_shortened_v3.tex <==
\section{Introduction} % all of page 1
% Code-switching (CS) is common in multi-cultural and multi-lingual societies, where speakers are bilingual and often switch between languages, such as Arabic-English, Hindi-English (Hinglish) and Spanish English (Spanglish), among many others, which can be seen as high-resource \textit{mono-language} in these language pairs \cite{ERR+18, HVA20}. In other cases like in South Africa, there are eleven spoken languages, of which Zulu and Xhosa are the most widely spoken, remarkably, in a single spoken utterance, a speaker may switch between Afrikaans, Xhosa and English \cite{reitmaier2022opportunities}. 

% modified by shammur


% The term 
Code-switching (CS) refers to the phenomenon where a speaker uses more than one language within the same discourse. \textcolor{blue}{CS is common in multi-cultural and multi-lingual societies, where speakers are bilingual and often switch between languages, such as Arabic-English, Hindi-English and Spanish-English, among many others.}
%In spontaneous speech, CS is very common and yet highly unpredictable and difficult to model. %With the advent of multilingualism, there has been an increasing interest in code-switching (CS) automatic speech recognition (ASR) \cite{SCR+19}. 

Automatic Speech Recognition (ASR) for CS is a well studied problem \cite{SCR+19} conducted in several language pairs on acoustic modeling, language modeling and novel system architectures. In code-switched language pairs with different scripts, there is a tendency to cross-transcribe words that creates a large number of homophones in the data, leading to challenges in training and evaluation. 
Rendering the CS transcription accurately is important, however, is often not straight-forward, and can be inconsistent, leading to the same word being transcribed using different scripts \cite{SS18}. Cross-transcription is particularly challenging in languages having a high amount of borrowing words, as it is not always clear which language a word belongs to, and hence, which script to transcribe it in. 
%Several socio-linguistic factors affect CS, due to which it is not uniform across language pairs \cite{dougruoz2021survey}. \cite{gamback2016comparing} define the Code-Mixing Index to measure the complexity of CS across languages and find that languages such as Nepali-English and Mandarin-English have a very high amount of switching compared to languages such as Dutch-Turkish in the Social Media corpora they study.
%placed here to appear on second page
\begin{table*}[h]
\centering
 \includegraphics[width=0.9\textwidth]{tables/fun_example_shortened-cropped.pdf}
 \label{table:fun_example}
 \caption{This example shows a hypothesis (H), the minimal edits annotation (ME), the ArzEn transcription reference (R), and their Buckwalter transliterations \cite{Buckwalter:2002:buckwalter} (R\_BW, H\_BW, and ME\_BW). We denote annotation decisions (A-Decision) as substitution (S), insertion (I), deletion (D), or acceptance (A) for words having different forms across H and ME. %We show CER/WER(ME,H) and CER/WER(R,H) reflecting the ground truth error of human post-editing as well as the CER and WER calculated between hypotheses and references. 
 In this example, CER and WER reductions are seen for minimal edits annotations over reference due to cross-transcription (segments 1, 2, 3, and 4) and unstandardized orthography (segments 9 and 13) issues. % (and unclear segment due to high speaking rate (segment 10)).
 }
 %\textcolor{red}{@Ahmed: Please let me know if this is okay or if you'd like to do it differently}}\textcolor{red}{@Amir: please explain what are ME, A, }
\end{table*}

Investigating the ideal ASR performance metric for CS, \cite{SS18} propose a modified WER metric based on mapping both languages into the pronunciation space, leading to improvements in accuracy and evaluation. \cite {ERR+18} propose a transliteration-based WER metric by transliterating mixed-script utterances into a single script. The authors demonstrate the robustness of the approach on several Indic languages. 
% keep it, if space allows, else commented
% \begin{comment}
Researchers have also investigated techniques for handling the problem of unstandardized orthography for Dialectal Arabic ASR evaluation. 
\cite{AMR15} propose the use of Multi-Reference Word Error Rate to allow for a wider coverage of different spelling variants for Dialectal Arabic ASR evaluation. 
Whereas, \cite{AKH19} investigate approaches to reduce spelling variations, which included normalization and following the Conventional Orthography for Dialectal Arabic (CODA) \cite{HDR12} guidelines to spell words, as well as relying on morphologically abstracted forms obtained from different tokenization schemes and lemmatization. 
% \end{comment}

Even though the aforementioned studies \cite {ERR+18,SS18} showed improved CS ASR performance, these techniques can also lead to false positives for words in the two languages that sound the same but have a different meaning. It also has limitation in cases where different part of the word written in different script. e.g, the word \textbf{\<آرت>ficial}, which is \textbf{artificial} in English script or \textbf{\<آرتفيشيال> } in Arabic script. 
Thanks to word-pieces \cite{chowdhury2021towards}, we may expect partial transcription in CS ASR results.

%Even though the aforementioned studies \cite {ERR+18,SS18} showed improved CS ASR performance %simple has not been recognized in English script  or Arabic script thanks to word-pieces, which may allows these cases in multi-lingual code-switching ASR results .

% Previous researchers have also investigated handling the problem of non-standardized orthography for Dialectal Arabic ASR evaluation. \cite{AMR15} proposed the use of Multi-Reference Word Error Rate to allow for a wider coverage of different spelling variants. \cite{AKH19} investigated approaches to reduce spelling variations, which included normalization and following the Conventional Orthography for Dialectal Arabic (CODA) \cite{HDR12} guidelines to spell words, as well as relying on morphologically abstracted forms obtained from different tokenization schemes and lemmatization.

This work builds upon previous contributions from \cite{SS18} and \cite{ERR+18}. In this study, we investigate various methods that go beyond orthographic transliteration methods. 
We explore lexical and phonetic representations for evaluation, and study various weighted edit-distance methods and semantic similarity evaluation. 
We designed a guideline and developed a reference human acceptability corpus (HAC) -- quantifying the human judgements in terms of minimal editing of ASR hypothesis. We evaluate a large number of metrics in correlation with human judgements. 
We believe that this is the first study on human acceptability for CS speech recognition. 

\noindent The contributions of this paper are as follows:
\setlength\itemsep{-0.1em}
\setlist[itemize]{noitemsep, topsep=-0.1pt}
\begin{itemize} %[noitemsep]

\item We design, develop and publicly release the first corpus for human acceptance for CS speech recognition;%\footnote{Data download link will be available upon paper acceptance.}

% \item We release the first corpus for human acceptance for code-switching speech recognition;%\footnote{Data download link will be available upon paper acceptance.}
\item We introduce phone similarity edit distance (PSD) and show its correlation with human acceptance;
\item We propose a novel approach to use machine translation on both hypotheses and references and report results using semantic evaluation to overcome the cross-transcription challenge.
\end{itemize}

\begin{comment}

* not all CS pairs are equal in complexity
* magic example
* challeneges of CS evaluation

* generalizability to other language pairs


\begin{figure}[t!]
    \centering
%    \includegraphics{}
\begin{tabular}{c|c}
     XXXX &  \\
     XXXX & \\
     XXXX &  \\
     XXXX & \\
     XXXX &  \\
     XXXX & \\
     
\end{tabular}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

%while WER is currently the de facto metric used for assessing speech recognition systems, several researchers have discussed its limitations \cite{}. Such limitations are further exacerbated in the case of code-switching, due to the possibility of code-switching segments to be written in either scripts, especially in the case of loanwords. In Figure/Table\ref{}, we show how CER and WER are both inadequate performance indicators, where many words and characters are incorrectly penalized, leading to a CER and WER that is double that achieved by human judgment.


\begin{figure}
  \includegraphics[width=\linewidth]{figures/cs_fun_example.png}
  \caption{(fun cs) Example demonstrating the difference between WER/CER and human assessment using minimal correction.}
  \label{fig:fun_cs}
\end{figure}
\end{comment}

%"researchers have argued the non-suitability of the WER metric for the evaluation of ASR systems for downstream tasks such as spoken language understanding (SLU) and information retrieval. The reason is that the WER works at the surface level and does not include any syntactic and semantic knowledge." \cite{Roy21}. Despite the great advances in ASR systems over the past year, "the means of evaluating the quality of a speech recognition system has remained mostly unchanged. WER is still the de facto standard metric for ASR system assessment."

==> sections/related_work.tex <==
\section{Related Work} %0.5 page;
%* Amir
%to be cited
Automatic Speech Recognition for Code-switching is a well studied problem \cite{SCR+19} with studies in several language pairs on acoustic modeling, language modeling and novel system architectures. In code-switched language pairs with different scripts, there is a tendency to cross-transcribe words leading to a large number of homophones in the data, leading to challenges in training and evaluation. Cross-transcription is particularly challenging in languages that have a high amount of borrowing, as it is not always clear which language a word belongs to. \cite{SS18} propose a modified WER metric based on mapping both languages into the pronunciation space, which leads to improvements in accuracy and evaluation. \cite {ERR+18} propose a transliteration-based WER metric by transliterating mixed-script utterances into a single script. However, these techniques can also lead to false positives when there are words in the two languages that sound the same but have a different meaning.

%(suggestion)Evaluation of dialectal Arabic-English CS ASR output is a challenging task as it combines the challenges of two worlds: dialectal Arabic and code-switching, in addition to the language-agnostic/universal challenges.
%\* Language-agnostic challenges include equal weight on different error types, literal comparisons without considering semantics.
%\* Challenges in DA has been previously investigated in \cite{AMR15,AKH19}. Multi-references to handle Unstandardization issues. Tokenization and lemmatization to handle morphological richness. 
%\* CS not much work done here. Work done by Sunayana on transliteration
%\* We point out that this is the first paper providing a benchmark for several evaluation metrics for CS ASR evaluation.

[MetricsMATR workshop..]


XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX

XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX XXXX 

==> tables/guidelines_example.tex <==
\subsection{Guidelines for Human judgments}
%Examples in a figure.
\begin{table*}[h]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ l r}
\hline
&\multicolumn{1}{c}{\textbf{MinEdits Examples}}\\\hline
Hypothesis&
\<ندين أكرم>
manuscript
\<بالإنجليش يعني مرة حاجة كت حاجة دي برضو كت ريليتد>
\\
MinEdits & 
the manuscript found in Accra
\<بالإنجليش يعني مرة حاجة كت حاجة برضو كت يعني ريليتد لتاريخ شوية اسمها>
\\\hline
Hypothesis&
\<بي إتش دي برة مصر بس ما اشتغلت في الأكاديمية>
dreaming of pursuing a masters egypt
\<بس أنا>\\
&
industry as research and development
\<أومين رول لا أبقى في>
as teaching my focus\\
MinEdits &
\<بي إتش دي برة مصر بس ما اشتغلش في ال أكاديميك>
egypt a 
\<في>
I'm dreaming of pursuing a masters 
\<بس يعني>
\\
&
industry as research and development
\<مين رول لا أبقى في ال >
my
\<أو>
my main focus 
\<يبقى>
as in teaching
\\\hline
\end{tabular}
\caption{Examples of minimal correction annotations task.[If time permits, I'll include only one example, showing what is accepted by humans and penalized by CER/WER.]}
\label{table:matchingAlg_examples}
\end{table*}

==> tables/old_results_sentenceLevel_correlations.tex <==
\begin{comment}
\begin{table*}[h]
\setlength{\tabcolsep}{2pt}
\begin{tabular}{|l|cc|cc|}
\cline{2-5}
\multicolumn{1}{c|}{}& \multicolumn{2}{c|}{Transliterating to Arabic}& \multicolumn{2}{c|}{Transliterating to English}\\
\hline
& CER(ref$_{TrAR}$,hyp$_{TrAr}$) & WER(ref$_{TrAR}$,hyp$_{TrAR}$) & CER(ref$_{TrEN}$,hyp$_{TrEN}$) & WER(ref$_{TrEN}$,hyp$_{TrEN}$) \\
\hline
CER(MinEdits,hyp) & 0.803& 0.372& 0.734& 0.527\\
WER(MinEdits,hyp) & 0.687& 0.441& 0.689& 0.608\\\hline    
\end{tabular}
\end{table*}

\begin{table*}[h]
\setlength{\tabcolsep}{1pt}
\begin{tabular}{|l|c|cc|cc|cc|}
\cline{3-8}
\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}& \multicolumn{2}{c|}{weight=2}& \multicolumn{2}{c|}{weight=4}& \multicolumn{2}{c|}{weight=8}\\\hline
& PER(ref,hyp) & PSD(ref,hyp) & PSD\_norm(ref,hyp) & PSD(ref,hyp) & PSD\_norm(ref,hyp) & PSD(ref,hyp) & PSD\_norm(ref,hyp) \\\hline
CER(MinEdits,hyp) & 0.7434& 0.767& 0.700& \textbf{0.774}& 0.734& 0.747& 0.732\\
WER(MinEdits,hyp) & 0.6478& 0.594& 0.497& \textbf{0.633}& 0.544& 0.636& 0.565\\\hline
\end{tabular}
\end{table*}

\begin{table*}[h]
\setlength{\tabcolsep}{2pt}
\begin{tabular}{|l|lll|lll|lll|lll|}
\hline
\multicolumn{1}{|c|}{}& \multicolumn{3}{c|}{Metric(ref$_{AR}$,hyp$_{AR}$)}  & \multicolumn{3}{c|}{Metric(ref$_{EN}$,hyp$_{EN}$)}   & \multicolumn{3}{c|}{Metric(ref$_{JA}$,hyp$_{JA}$)}   & \multicolumn{3}{c|}{Average} \\
\cline{2-13}
\multicolumn{1}{|c|}{}& BLEU   & chrF  & Sem    & BLEU   & chrF   & Sem    & BLEU   & chrF   & Sem    & BLEU    & chrF    & Sem     \\
\hline
CER(MinEdits,hyp) & 0.25 & 0.55 & 0.64 & 0.49 & 0.62 & 0.60 & 0.45 & 0.49 & 0.59 & 0.50  & 0.65  & 0.72  \\
WER(MinEdits,hyp) & 0.32 & 0.52 & 0.59 & 0.54 & 0.65 & 0.61 & 0.48 & 0.53 & 0.53 & 0.56  & 0.67  & 0.68\\\hline
%CORREL(CER(HME,hyp),metric(ref,hyp)) & 0.253 & 0.551 & 0.640 & 0.492 & 0.622 & 0.601 & 0.447 & 0.492 & 0.591 & 0.499  & 0.649  & 0.716  \\
%CORREL(WER(HME,hyp),metric(ref,hyp)) & 0.322 & 0.519 & 0.586 & 0.542 & 0.650 & 0.610 & 0.482 & 0.535 & 0.526 & 0.558  & 0.667  & 0.679 
\end{tabular}
\end{table*}

\begin{table*}[h]
\setlength{\tabcolsep}{0.9pt}
\begin{tabular}{|l|ccc|cccc|}
\hline
& CER(ref,hyp) & WER(ref,hyp) & MER(ref,hyp) & Transliteration & PhoneticSimilarity & SemanticSimilarity &
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Average(\\ Transliteration,\\ PhoneticSimilarity,\\ SemanticSimilarity)\end{tabular}} \\\hline
CER(MinEdits,hyp) & 0.683& 0.372& 0.445& 0.803& 0.774& 0.716& \textbf{0.820}\\
WER(MinEdits,hyp) & 0.622& 0.437                            & 0.516& 0.687& 0.633& 0.680& \textbf{0.703}\\\hline
\end{tabular}
\end{table*}
\end{comment}

==> tables/phonological_similarity_example.tex <==
\begin{table*}[ht!]
\setlength{\tabcolsep}{1pt}
\begin{tabular}{l p{4cm} | r r}
\hline
\multicolumn{1}{c}{}&\multicolumn{1}{c}{Text}& PER & PSD\\\hline
R&
\multicolumn{1}{l}{
i have to say 
\<اخر سفرية لي اللي هي في المانيا علشان اشتغلت فيها كويس اوي و كانت يعني كانت>
very fruitful
} & & \\
H&
\multicolumn{1}{l}{
 
 \<أي هفتو ساي آخر سفرية ليا اللي هي في ألمانيا علشان اشتغلت فيها كويس قوي وكانت يعني كانت>
 very fruit\<فل>
 }
 &&\\\hline
R$_{phone}$& 
\multicolumn{1}{l}{aj hæv tə sej axr sfrit li alli hi fi almania ʕlʃan aʃtɣlt fiha kuis aui u kant iʕni kant vɛɹi fɹutfəl}
&  &  \\
H$_{phone}$&
\multicolumn{1}{l}{ai hftu sai aٓxr sfrit lia alli hi fi almania ʕlʃan aʃtɣlt fiha kuis qui ukant iʕni kant vɛɹi fɹutfl}
& 0.12 & 0.10\\\hline
\end{tabular}
\caption{Example showing IPA phone mapping for the reference (R) and hypothesis (H) using Epitran with phone PER and PSD error rates.}
\label{table:PSDexample}
\end{table*}

==> tables/results_sentenceLevel_correlations.tex <==
\begin{table*}[ht]
  \centering
  \medskip
  \setlength{\tabcolsep}{1pt}
  \begin{tabularx}{\linewidth}{p{2.5cm} X X X X X X X X}
    \toprule
    \multicolumn{9}{c}{\textbf{Orthographic Metrics}} \\
    \midrule
     %&  &  &  &  & \multicolumn{4}{c}{Transliteration}\\\cmidrule(lr){6-9}
     & WER & MER & WIL & CER & WER$^{TrAR}$ & CER$^{TrAR}$ & CER$^{TrEN}$ & CER$^{TrEN}$\\
    %\midrule
    \cmidrule(lr){2-9}
    CER(ME,hyp) & x &  &  &  &  &  &  & \\
    WER(ME,hyp) & x &  &  &  &  &  &  & \\
    \midrule
  \end{tabularx}
  \begin{tabularx}{\linewidth}{ p{2.5cm} X X X X X X X}
    \multicolumn{8}{c}{\textbf{Phonological Metrics}} \\
    \midrule
     & PER & PSD$_{w=2}$ & PSD\_norm$_{w=2}$ & PSD$_{w=4}$ & PSD\_norm$_{w=4}$ & PSD$_{w=8}$ & PSD\_norm$_{w=8}$\\
    %\midrule
    \cmidrule(lr){2-8}
    CER(ME,hyp) & x &  &  &  &  &  & \\
    WER(ME,hyp) & x &  &  &  &  &  & \\ 
    \bottomrule
  \end{tabularx}
  \begin{tabularx}{\linewidth}{ p{2.5cm} X X X X X X X X X X X X X X X}
    \multicolumn{11}{c}{\textbf{Semantic Metrics}} \\
    \midrule
     %& \multicolumn{5}{c}{Original Text} & \multicolumn{5}{c}{Arabic Translation} \\\cmidrule(lr){2-6}\cmidrule(lr){7-11}
     & BLEU$^{CS}$ & chrF$^{CS}$ & B(F1)$^{CS}$ & $Sim_{CLS}^{CS}$ & $Sim_{MP}^{CS}$ & BLEU$^{AR}$ & chrF$^{AR}$ & B(F1)$^{AR}$ & $Sim_{CLS}^{AR}$ & $Sim_{MP}^{AR}$ \\
    %\midrule
    \cmidrule(lr){2-11}
    CER(ME,hyp) & x &  &  &  &  &  & \\
    WER(ME,hyp) & x &  &  &  &  &  & \\ 
    %& \multicolumn{5}{c}{Original Text} & \multicolumn{5}{c}{Arabic Translation} \\\cmidrule(lr){2-6}\cmidrule(lr){7-11}
     & BLEU$^{EN}$ & chrF$^{EN}$ & B(F1)$^{EN}$ & $Sim_{CLS}^{EN}$ & $Sim_{MP}^{EN}$ & BLEU$^{JA}$ & chrF$^{JA}$ & B(F1)$^{JA}$ & $Sim_{CLS}^{JA}$ & $Sim_{MP}^{JA}$ \\
    %\midrule
    \cmidrule(lr){2-11}
    CER(ME,hyp) & x &  &  &  &  &  & \\
    WER(ME,hyp) & x &  &  &  &  &  & \\ 
    & &&BLEU$^{AV}$ & chrF$^{AV}$ & B(F1)$^{AV}$ & $Sim_{CLS}^{AV}$ & $Sim_{MP}^{AV}$ \\
    %\midrule
    \cmidrule(lr){2-11}
    CER(ME,hyp) &&& x &  &  &  &  &  & \\
    WER(ME,hyp) &&& x &  &  &  &  &  & \\ 
    \bottomrule
  \end{tabularx}
  \caption{Sentence-level correlations.}
  \label{tbl:interesting}
\end{table*}

==> tables/translation_similarity_example.tex <==
\begin{table*}[t]
\begin{tabular}{|l|r|ccc|}
\hline
&& BLEU& chrF& Semantic Similarity\\\hline
hyp& 
\<آ ده أغلب ال أكتفيتيز اللي أنا بعملها في الجامعة يعني>
& & & 0.7722              \\
ref& 
\<ده اغلب ال>
 activities
 \<اللى انا بعملها فى الجامعة يعنى>&&&\\\hline
hyp\_ar & 
\<آ ده أغلب ال أكتفيتيز اللي أنا بعملها في الجامعة يعني>
& 4.9  & 49.6 & 0.8740               \\
ref\_ar &
\<أنشطة ده اغلب اللى انا بعملها فى الجامعة يعنى>&&&\\\hline
hyp\_en & \multicolumn{1}{l|}{Oh, this is most of the activeties that I do at university, I mean} & 22.9 & 65.4 & 0.8665\\
ref\_en & \multicolumn{1}{l|}{These are most of the activities that I do at the university}&&&\\\hline
hyp\_ja & \multicolumn{1}{l|}{\begin{CJK}{UTF8}{min}ああ、これは私が大学で行っている活動のほとんどです、つまり\end{CJK}}& 67.5 & 82.6 & 0.9581\\
ref\_ja & \multicolumn{1}{l|}{\begin{CJK}{UTF8}{min}これらは私が大学で行っている活動のほとんどです\end{CJK}}&&&\\\hline
\end{tabular}
\end{table*}

==> tables/transliteration_example.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l p{5cm} l l}
\hline
\multicolumn{1}{c}{}&\multicolumn{1}{c}{Text}& CER& WER\\\hline
R&
\multicolumn{1}{c}{
manuscript found in acra
\<كان اسمه>
} & 30.3 & 66.7 \\
H&
\multicolumn{1}{c}{
 \<أكره>
 manuscript found an 
 \<ياعصمه>}
 &&\\\hline
R$_{TrAr}$& 
\multicolumn{1}{l}{\<كان اسمه مانوسكريبت فوند ين اكرا>}
& 25.9 & 66.7 \\
H$_{TrAr}$&
\multicolumn{1}{l}{\<ياعصمه مانوسكريبت فوند ان أكره>}
&&\\\hline
R$_{TrEn}$& 
\multicolumn{1}{l}{Kan Asmah manuscript found in acra} & 27.6 & 66.7 \\
H$_{TrEn}$& 
\multicolumn{1}{l}{easme manuscript found an Aqrah}    &&\\\hline
\end{tabular}
\caption{Transliteration example showing the CER and WER for calculated for the reference (R) and hypothesis (H) with and without transliteration.\textcolor{red}{(can we find another ex., where CER and WER move closer towards minEdits?)}}
\label{table:transliteration_example}
\end{table}
